Privacy- and Utility-Preserving NLP with Anonymized Data: A case study of Pseudonymization

This work investigates the effectiveness of different pseudonymization techniques, ranging from rule-based substitutions to using pre-trained Large Language Models (LLMs), on a variety of datasets and models used for two widely used NLP tasks: text classification and summarization. Our work provides crucial insights into the gaps between original and anonymized data (focusing on the pseudonymization technique) and model quality and fosters future research into higher-quality anonymization techniques to better balance the trade-offs between data protection and utility preservation. We make our code, pseudonymized datasets, and downstream models publicly available

==> tab/classification.tex <==
\begin{table}[t]
\centering
\tiny
\begin{tabular}{p{0.30\linewidth} | p{0.25\linewidth}}
\toprule
 & \textbf{F-score} \\ 
 \midrule
\textbf{Original text} & \textbf{88.42} \\
\midrule
\textbf{NER-Sanit\textsubscript{(SPACY)}} &  87.65 \textcolor{red}{(-0.77)} \\ 
\textbf{NER-Sanit\textsubscript{(FLAIR)}} & 87.88 \textcolor{red}{(-0.54)} \\ 
\midrule
\textbf{NER-PS\textsubscript{(SPACY)}} &  88.06 \textcolor{red}{(-0.36)} \\ 
\textbf{NER-PS\textsubscript{(FLAIR)}} &  88.14 \textcolor{red}{(-0.28)} \\ 
\midrule
\textbf{Seq2Seq-PS\textsubscript{(SPACY)}}) & 88.10 \textcolor{red}{(-0.32)} \\
\textbf{Seq2Seq-PS\textsubscript{(FLAIR)}} & 88.13 \textcolor{red}{(-0.29)} \\ 
\midrule
\textbf{LLM-PS} & 88.15 \textcolor{red}{(-0.27)} \\ 
\bottomrule
\end{tabular}
\caption{Results of text classification downstream task. \textcolor{red}{<need to replace constant  colors with colormap>}}
\label{table-text-classification-results}
\end{table}

==> tab/sum_classif2.tex <==
\begin{table}[t]
\tiny
 %\begin{tabular}{p{0.10\linewidth}p{0.10\linewidth}|p{0.10\linewidth}|p{0.10\linewidth}||p{0.1\linewidth}}
\begin{booktabs}{
  colspec = {l|ccc|c},
  cell{1}{4} = {c=1}{c}, % multicolumn (column number=2, center alignment)
  cell{1}{2} = {c=3}{c} % multicolumn (column number=2, center alignment)
}
\toprule
& \textbf{Summarization} & & & \textbf{Classification} \\
\cmidrule[lr]{2-4}\cmidrule[lr]{5-5}
& \textbf{ROUGE-1} & \textbf{ROUGE-2} & \textbf{ROUGE-L} & \textbf{F-score} \\
 \midrule
\textbf{Original text} & \textbf{42.82} &  \textbf{20.13} &  \textbf{36.33} & \textbf{88.42} \\
\midrule
\textbf{{NER-S}\textsubscript{(SPACY)}} &   41.59 \xatext{(-1.23)} &  19.17 \aatext{(-0.96)} & 29.07 \batext{(-7.26)}  & 87.65  \catext{(-0.77)} \\
\textbf{NER-S\textsubscript{(FLAIR)}} & 39.05 \xbtext{(-3.77)} &  17.52 \abtext{(-2.61)} & 27.43 \bbtext{(-8.90)} &  87.88 \cbtext{(-0.54)} \\
\midrule
\textbf{NER-PS\textsubscript{(SPACY)}} &  41.93 \xctext{(-0.89)} &  19.38 \actext{(-0.75)} &  29.36 \bctext{(-6.97)} & 88.06 \cctext{(-0.36)}\\
\textbf{NER-PS\textsubscript{(FLAIR)}} &  40.25 \xdtext{(-2.57)} &  18.04 \adtext{(-2.09)} & 27.97 \bdtext{(-8.36)} & 88.14 \cdtext{(-0.28)} \\
\midrule
\textbf{S2S-PS\textsubscript{(SPACY)}} & 39.1 \xetext{(-3.82)} & 17.23 \aetext{(-2.90)} & 26.96 \betext{(-9.37)} & 88.10 \cetext{(-0.32)} \\
\textbf{S2S-PS\textsubscript{(FLAIR)}} & 36.04\xftext{(-6.78)}& 15.07\aftext{(-5.06)}&24.73\bftext{(-11.6)}& 88.13 \cftext{(-0.29)} \\
\midrule
\textbf{LLM-PS} & 38.62 \xgtext{(-4.20)} & 16.57 \agtext{(-3.56)} & 26.34 \bgtext{(-9.99)} & 88.15 \cftext{(-0.27)}\\
\bottomrule
\end{booktabs}
%\end{tabular}
\caption{Results of downstream evaluation tasks: summarization (left) and text classification (right). The smaller the gap with the original text, the better the utility is preserved.}
%\textcolor{red}{<need to replace constant colors with colormap>}
\label{table-summarization-results}
\end{table}

